BackFlip: The Impact of Local and Global Data Augmentations on Artistic Image Aesthetic Assessment

Assessing the aesthetic quality of artistic images presents unique challenges due to the subjective nature of aesthetics and the complex visual characteristics inherent to artworks. Basic data augmentation techniques commonly applied to natural images in computer vision may not be suitable for art images in aesthetic evaluation tasks, as they can change the composition of the art images. In this paper, we explore the impact of local and global data augmentation techniques on artistic image aesthetic assessment (IAA). We introduce BackFlip, a local data augmentation technique designed specifically for artistic IAA. We evaluate the performance of BackFlip across three artistic image datasets and four neural network architectures, comparing it with the commonly used data augmentation techniques. Then, we analyze the effects of components within the BackFlip pipeline through an ablation study. Our findings demonstrate that local augmentations, such as BackFlip, tend to outperform global augmentations on artistic IAA in most cases, probably because they do not perturb the composition of the art images. These results emphasize the importance of considering both local and global augmentations in future computational aesthetics research.

==> results_BAID_tmp.tex <==
\begin{table}[ht!]
\fontsize{7}{9}\selectfont

\begin{tabular}{ll|lll}
& \multirow{2}{*}{\textbf{Augmentation}} & \multicolumn{3}{c}{\textbf{BAID}} \\
\multicolumn{1}{c}{} &  & \textbf{Acc. (\%)} & \textbf{PCC} & \textbf{SRCC} \\
\midrule 

\multirow{9}{*}{\rotatebox[origin=c]{90}{\textbf{ResNet-18}}} & Resize, Center Crop & $ 74.93 \pm 1.6 $ & $ 0.41 \pm 0.04 $ & $ 0.29 \pm 0.04 $ \\
 & Resize, Random Crop & $ 70.24 \pm 3.81 $ & $ 0.3 \pm 0.03 $ & $ 0.22 \pm 0.02 $ \\
 & Random Resized Crop & $ 71.71 \pm 4.71 $ & $ 0.3 \pm 0.07 $ & $ 0.27 \pm 0.06 $ \\
 & Resize, Center Crop, Horizontal flip &  $ 70.31 \pm 1.6 $ & $ 0.31 \pm 0.03 $ & $ 0.21 \pm 0.02 $ \\
 & Resize, Center Crop, Vertical flip &  $ 70.04 \pm 4.09 $ & $ 0.31 \pm 0.02 $ & $ 0.22 \pm 0.02 $ \\
 & Resize, Center Crop, Rotation &  $ 70.93 \pm 1.94 $ & $ 0.31 \pm 0.03 $ & $ 0.23 \pm 0.03 $ \\
 & Resize, Center Crop, Erase+Inpaint & $\mathit{ 74.9 \pm 1.05 }$ & $\mathit{ 0.4 \pm 0.02 }$ & $\mathit{ 0.27 \pm 0.03 }$ \\
 & Resize, Center Crop, BoxFlip & $ 71.01 \pm 3.19 $ & $ 0.37 \pm 0.03 $ & $ 0.22 \pm 0.06 $ \\
 & Resize, Center Crop, BackFlip & $\mathit{ 71.5 }$ & $\mathit{ 0.32 }$ & $\mathit{ 0.22 }$ \\
\midrule 


\multirow{9}{*}{\rotatebox[origin=c]{90}{\textbf{ResNet-50}}} & Resize, Center Crop & $ 70.14 \pm 1.88 $ & $ 0.29 \pm 0.05 $ & $ 0.2 \pm 0.05 $ \\
 & Resize, Random Crop & $ 72.29 \pm 1.26 $ & $ 0.29 \pm 0.04 $ & $ 0.22 \pm 0.03 $ \\
 & Random Resized Crop & $ 72.58 \pm 5.64 $ & $ 0.28 \pm 0.08 $ & $ 0.25 \pm 0.05 $ \\
 & Resize, Center Crop, Horizontal flip & $ 71.15 \pm 5.7 $ & $ 0.32 \pm 0.05 $ & $ 0.24 \pm 0.05 $ \\
 & Resize, Center Crop, Vertical flip &  $ 72.17 \pm 0.85 $ & $ 0.33 \pm 0.05 $ & $ 0.25 \pm 0.05 $ \\
 & Resize, Center Crop, Rotation & $ 71.69 \pm 4.84 $ & $ 0.3 \pm 0.01 $ & $ 0.24 \pm 0.02 $ \\
 & Resize, Center Crop, Erase+Inpaint & $\mathit{ 72.41 \pm 5.07 }$ & $\mathit{ 0.36 \pm 0.05 }$ & $\mathit{ 0.26 \pm 0.04 }$ \\
 & Resize, Center Crop, BoxFlip & $ 74.02 \pm 0.6 $ & $ 0.38 \pm 0.02 $ & $ 0.24 \pm 0.02 $ \\
 & Resize, Center Crop, BackFlip & $\mathit{ 73.68 \pm 4.11 }$ & $\mathit{ 0.36 \pm 0.05 }$ & $\mathit{ 0.25 \pm 0.03 }$ \\
\midrule 


\multirow{9}{*}{\rotatebox[origin=c]{90}{\textbf{ResNeXt50}}} & Resize, Center Crop &  $ 73.3 \pm 3.13 $ & $ 0.37 \pm 0.05 $ & $ 0.27 \pm 0.02 $ \\
 & Resize, Random Crop & $ 74.49 \pm 1.03 $ & $ 0.32 \pm 0.09 $ & $ 0.25 \pm 0.09 $ \\
 & Random Resized Crop & $ 75.13 \pm 2.33 $ & $ 0.3 \pm 0.13 $ & $ 0.32 \pm 0.04 $ \\
 & Resize, Center Crop, Horizontal flip & $ 73.48 \pm 0.82 $ & $ 0.34 \pm 0.05 $ & $ 0.25 \pm 0.04 $ \\
 & Resize, Center Crop, Vertical flip &  $ 72.6 \pm 1.65 $ & $ 0.3 \pm 0.02 $ & $ 0.23 \pm 0.01 $ \\
 % & Resize, Center Crop, Rotation &  &  &  \\
 & Resize, Center Crop, Erase+Inpaint &   $\mathit{ 74.28 \pm 0.28 }$ & $\mathit{ 0.37 \pm 0.02 }$ & $\mathit{ 0.25 \pm 0.01 }$ \\
 & Resize, Center Crop, BoxFlip & $ 73.93 \pm 1.35 $ & $ 0.35 \pm 0.03 $ & $ 0.23 \pm 0.02 $ \\
 & Resize, Center Crop, BackFlip &  $\mathit{ 74.75 \pm 0.52 }$ & $\mathit{ 0.35 \pm 0.02 }$ & $\mathit{ 0.23 \pm 0.02 }$ \\
\midrule 


\multirow{9}{*}{\rotatebox[origin=c]{90}{\textbf{SAAN}}} & Resize, Center Crop & $ 74.77 \pm 1.37 $ & $ 0.37 \pm 0.03 $ & $ 0.3 \pm 0.04 $ \\
 & Resize, Random Crop & $ 72.4 \pm 1.16 $ & $ 0.37 \pm 0.03 $ & $ 0.29 \pm 0.03 $ \\
 & Random Resized Crop & $ 76.46 \pm 0.37 $ & $ 0.41 \pm 0.03 $ & $ 0.37 \pm 0.02 $ \\
 & Resize, Center Crop, Horizontal flip & $\mathit{ 71.02 \pm 1.77 }$ & $\mathit{ 0.32 \pm 0.01 }$ & $\mathit{ 0.26 \pm 0.01 }$ \\
 
 & Resize, Center Crop, Vertical flip & $ 73.95 \pm 0.8 $ & $ 0.35 \pm 0.02 $ & $ 0.3 \pm 0.03 $ \\
 % & Resize, Center Crop, Rotation &  &  &  \\
 & Resize, Center Crop, Erase+Inpaint &  $\mathit{ 74.19 \pm 1.15 }$ & $\mathit{ 0.41 \pm 0.03 }$ & $\mathit{ 0.31 \pm 0.05 }$ \\
 & Resize, Center Crop, BoxFlip &  $ 73.27 \pm 1.74 $ & $ 0.37 \pm 0.04 $ & $ 0.29 \pm 0.03 $ \\
 & Resize, Center Crop, BackFlip & $\mathit{ 74.41 \pm 0.98 }$ & $\mathit{ 0.4 \pm 0.01 }$ & $\mathit{ 0.33 \pm 0.03 }$ \\
\midrule 

\end{tabular}
\caption{Results on BAID for four computer vision models trained with different image data augmentation techniques. 
The \textit{Italic} font is used to indicate preliminary results. 
In the rest of the table, we report the average accuracy across at least 5 independent runs. The complete results will be provided in the final submission. \todo{Update table with the final results.}
% \om{I will add all the results when I have 5 runs for each row.} \om{Not sure what is the best way to visualize the results. Maybe the histograms are easier to read. }
\\
\om{
ResNet18: 50 epochs, 256 batch size, lr 0.001, Adam \\
ResNet50: 50 epochs, 512 batch size, lr 0.001, Adam \\
ResNext: 50 epochs, 256 batch size, lr 0.001, Adam \\
SAAN: 50 epochs, 256 batch size, lr 0.0001, AdamW \\
Setup for Backflip/Erase+Inp.: median inpainting, 3 augmented segments, hor./ver. flip. \\
All models are pretrained on ImageNet. 
}
}
\label{tab:BAID_results}
\end{table}
